How Much Can D2D Communication Reduce Content Delivery Latency in Fog Networks with Edge Caching?

A Fog-Radio Access Network (F-RAN) is studied in which cache-enabled Edge Nodes (ENs) with dedicated fronthaul connections to the cloud aim at delivering contents to mobile users. Using an information-theoretic approach, this work tackles the problem of quantifying the potential latency reduction that can be obtained by enabling Device-to-Device (D2D) communication over out-of-band broadcast links. Following prior work, the Normalized Delivery Time (NDT) --- a metric that captures the high signal-to-noise ratio worst-case latency --- is adopted as the performance criterion of interest. Joint edge caching, downlink transmission, and D2D communication policies based on compress-and-forward are proposed that are shown to be information-theoretically optimal to within a constant multiplicative factor of two for all values of the problem parameters, and to achieve the minimum NDT for a number of special cases. The analysis provides insights on the role of D2D cooperation in improving the delivery latency.

==> packages_commands_theorems.tex <==

\usepackage[utf8]{inputenc} 


\usepackage[T1]{fontenc}


\usepackage{cite}


\ifCLASSINFOpdf
 \usepackage[pdftex]{graphicx}
 \graphicspath{{../pdf/}{../jpeg/}}
 \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\else
 \usepackage[dvips]{graphicx}
 \graphicspath{{../eps/}}
 \DeclareGraphicsExtensions{.eps}
\fi


\usepackage[cmex10]{amsmath}  
\usepackage{amssymb}
\interdisplaylinepenalty=2500 



\usepackage{algorithmic}


\usepackage{array}




\usepackage{stfloats}

\usepackage{flafter}


\usepackage{url}


\usepackage{cases}


\usepackage{tikz}
\usetikzlibrary{calc} % calculation of coordinates
\usepackage{pgfplots}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning}
\usetikzlibrary{arrows.meta} % change arrow tip
\usetikzlibrary{shapes} % for shapes



\RequirePackage{microtype}


\usepackage{xcolor}
\definecolor{TechnionBlue}{rgb}{0, 0.1765, 0.3843} % Technion Blue color
\definecolor{OliveGreen}{rgb}{0.4, 0.62, 0.25} % Olive Green color


\usepackage{ifthen}

\newcommand{\rb}[1] {\left(#1\right)}
\newcommand{\cb}[1] {\left\lbrace #1 \right\rbrace}
\newcommand{\sqb}[1] {\left[#1\right]}
\newcommand{\given}[1]{\left\lvert#1\right.}
\newcommand{\AgivenB}[2]{\left(#1\middle\vert#2\right)}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}
\newcommand*{\nspace}[1] {
	\ifthenelse{\equal{#1}{!}}{\!}{} % thin negative space
	\ifthenelse{\equal{#1}{tq}}{\kern-1em}{} % In text mode: \kern-1em equals "minus quad"
	\ifthenelse{\equal{#1}{mq}}{\mkern-18mu}{} % In math mode: \mkern-18mu equals "minus quad"
}

\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
